Selecting Walk Schemes for Database Embedding

Machinery for data analysis often requires a numeric representation of the input. Towards that, a common practice is to embed components of structured data into a high-dimensional vector space. We study the embedding of the tuples of a relational database, where existing techniques are often based on optimization tasks over a collection of random walks from the database. The focus of this paper is on the recent FoRWaRD algorithm that is designed for dynamic databases, where walks are sampled by following foreign keys between tuples. Importantly, different walks have different schemas, or "walk schemes", that are derived by listing the relations and attributes along the walk. Also importantly, different walk schemes describe relationships of different natures in the database. We show that by focusing on a few informative walk schemes, we can obtain tuple embedding significantly faster, while retaining the quality. We define the problem of scheme selection for tuple embedding, devise several approaches and strategies for scheme selection, and conduct a thorough empirical study of the performance over a collection of downstream tasks. Our results confirm that with effective strategies for scheme selection, we can obtain high-quality embeddings considerably (e.g., three times) faster, preserve the extensibility to newly inserted tuples, and even achieve an increase in the precision of some tasks.

==> plots/dynamic/HepatitisDynamic.tex <==
\begin{tikzpicture}
\begin{axis}[
    title={Hepatitis},
    width=7.5cm,
    height=4.5cm,
    xlabel={Ratio of new data (\%)},
    ylabel={Accuracy (\%)},
    xmin=5, xmax=95,
    ymin=0, ymax=105,
    xtick={10,20,30,40,50,60,70,80,90},
    ytick={0,20,40,60,80,100},
    xtick pos=left,
    ytick pos=left,
    y label style={at={(axis description cs:0.12,0.5)},anchor=south},
    legend style={at={(1.05,0.5)},anchor=west},
    ymajorgrids=true,
    grid style=dashed,
]

\addplot[
    color=gray,
    mark=square,
    ]
    coordinates {
    (10,92.6)(20,91)(30,92.22)(40,89.65)(50,87.16)(60,85.47)(70,81.89)(80,75.45)(90,68.04)
    };
    

\addplot[
    color=red,
    mark=o,
    ]
    coordinates {
    (10,84.2)(20,84.9)(30,83.87)(40,82.75)(50,79.96)(60,79.33)(70,78.26)(80,75.92)(90,72.02)
    };


\addplot[
    color=blue,
    mark=triangle,
    ]
    coordinates {
    (10,73.6)(20,73.6)(30,75.07)(40,74.9)(50,74.72)(60,75.47)(70,74.74)(80,75.25)(90,69.73)
    };

\addplot[
    color=black,
    ]
    coordinates {
    (5,58.8)(95,58.8)
    };
    
%\legend{Node2Vec, FoRWaRD, Baseline}
    
\end{axis}
\end{tikzpicture}


==> plots/mega_figure.tex <==
\begin{figure*}
\ifx\QUICK\undefined
%begin 1 world
\centering
\rotatebox[origin=t]{90}{\small~\textbf{world}}
\begin{subfigure}{0.155\textwidth}
    \caption*{\textbf{k\_var}}
    %\includegraphics[width=\textwidth]{plots/world_k_var.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/world_k_var.tex}}
    %\caption{Time}
    \label{fig:first}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    \caption*{\textbf{MI}}
    %\includegraphics[width=\textwidth]{plots/world_ent.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/world_MI.tex}}
    %\caption{Time}
    \label{fig:second}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    \caption*{\textbf{1ep}}
    %\includegraphics[width=\textwidth]{plots/world_1ep.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/world_1ep.tex}}
    %\caption{Time}
    \label{fig:third}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    \caption*{\textbf{len}}
    %\includegraphics[width=\textwidth]{plots/world_len.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/world_len.tex}}
    %\caption{Time}
    \label{fig:third4}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    \caption*{\textbf{random}}
    %\includegraphics[width=\textwidth]{plots/world_random.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/world_random.tex}}
    %\caption{Time}
    \label{fig:third5}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    \caption*{\textbf{random}}
    %\includegraphics[width=\textwidth]{plots/world_sampling.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/world_sampling.tex}}
    %\caption{Time}
    \label{fig:third6}
\end{subfigure}
%end 1 world






%begin 2 genes
\centering
\rotatebox[origin=t]{90}{\small~\textbf{genes}}
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/genes_k_var.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/genes_k_var.tex}}
    %\label{fig:first}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/genes_ent.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/genes_MI.tex}}
    %\label{fig:second}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/genes_1ep.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/genes_1ep.tex}}
    %\label{fig:third}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/genes_len.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/genes_len.tex}}
    %\label{fig:third4}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/genes_random.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/genes_random.tex}}
    %\label{fig:third5}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/genes_sampling.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/genes_sampling.tex}}
    %\label{fig:third6}
\end{subfigure}
%end 2 genes






%begin 3 mondial_religion
\centering
\rotatebox[origin=t]{90}{\small~\textbf{M religion}} %Acc-mondial_religion
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_religion_k_var.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_religion_k_var.tex}}
    %\label{fig:first}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_religion_ent.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_religion_MI}}
    %\label{fig:second}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_religion_1ep.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_religion_1ep.tex}}
    %\label{fig:third}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_religion_len.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_religion_len.tex}}
    %\label{fig:third4}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_religion_random.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_religion_random.tex}}
    %\label{fig:third5}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_religion_sampling.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_religion_sampling.tex}}
    %\label{fig:third6}
\end{subfigure}
%end 3 mondial_religion






%begin 4 mondial_continent
\centering
\rotatebox[origin=t]{90}{\small~\textbf{M continent}} %
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_continent_k_var.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_continent_k_var.tex}}
    %\label{fig:first}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_continent_ent.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_continent_MI}}
    %\label{fig:second}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_continent_1ep.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_continent_1ep.tex}}
    %\label{fig:third}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_continent_len.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_continent_len.tex}}
    %\label{fig:third4}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_continent_random.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_continent_random.tex}}
    %\label{fig:third5}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_continent_random.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_continent_sampling.tex}}
    %\label{fig:third6}
\end{subfigure}
%end 4 mondial_continent






%begin 5 mondial_inflation
\centering
\rotatebox[origin=t]{90}{\small~\textbf{M inflation}} %Acc-mondial_inflation
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_inflation_k_var.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_inflation_k_var.tex}}
    %\label{fig:first}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_inflation_ent.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_inflation_MI}}
    %\label{fig:second}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_inflation_1ep.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_inflation_1ep.tex}}
    %\label{fig:third}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_inflation_len.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_inflation_len.tex}}
    %\label{fig:third4}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_inflation_random.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_inflation_random.tex}}
    %\label{fig:third5}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_inflation_sampling.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_inflation_sampling.tex}}
    %\label{fig:third6}
\end{subfigure}
%end 5 mondial_inflation






%begin 6 hepatitis
\centering
\rotatebox[origin=t]{90}{\small~\textbf{hepatitis}}
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/hepatitis_k_var.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/hepatitis_k_var.tex}}
    %\label{fig:first}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/hepatitis_ent.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/hepatitis_MI}}
    %\label{fig:second}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/hepatitis_1ep.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/hepatitis_1ep.tex}}
    %\label{fig:third}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/hepatitis_len.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/hepatitis_len.tex}}
    %\label{fig:third4}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/hepatitis_random.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/hepatitis_random.tex}}
    %\label{fig:third5}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/hepatitis_sampling.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/hepatitis_sampling.tex}}
    %\label{fig:third6}
\end{subfigure}
%end 6 hepatitis






%begin 7 mondial_infant-mortality
\centering
\rotatebox[origin=t]{90}{\small~\textbf{M infant-mort.}} %Acc-mondial_infant-mortality
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_infant-mortality_k_var.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_infant-mortality_k_var.tex}}
    %\label{fig:first}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_infant-mortality_ent.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_infant-mortality_MI}}
    %\label{fig:second}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_infant-mortality_1ep.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_infant-mortality_1ep.tex}}
    %\label{fig:third}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_infant-mortality_len.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_infant-mortality_len.tex}}
    %\label{fig:third4}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_infant-mortality_random.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_infant-mortality_random.tex}}
    %\label{fig:third5}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_infant-mortality_sampling.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_infant-mortality_sampling.tex}}
    %\label{fig:third6}
\end{subfigure}
%end 7 mondial_infant-mortality






%begin 8 mondial_GDP
\centering
\rotatebox[origin=t]{90}{\small~\textbf{M GDP}} %Acc-mondial_GDP
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_GDP_k_var.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_GDP_k_var.tex}}
    %\label{fig:first}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_GDP_ent.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_GDP_MI}}
    %\label{fig:second}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_GDP_1ep.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_GDP_1ep.tex}}
    %\label{fig:third}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_GDP_len.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_GDP_len.tex}}
    %\label{fig:third4}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_GDP_random.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_GDP_random.tex}}
    %\label{fig:third5}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_GDP_sampling.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_GDP_sampling.tex}}
    %\label{fig:third6}
\end{subfigure}
%end 8 mondial_GDP







%begin 9 last mutagenesis
\rotatebox[origin=t]{90}{\small~\textbf{mutagenesis}} 
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mutagenesis_k_var.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mutagenesis_k_var.tex}}
    \caption*{\textbf{Time} (sec)}
    \label{fig:2first}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mutagenesis_1ep.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mutagenesis_1ep.tex}}
    \caption*{\textbf{Time} (sec)}
    \label{fig:2second}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/empty.png}  % mutagenesis_entropy
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mutagenesis_MI}}
    \caption*{\textbf{Time} (sec)}
    \label{fig:2third}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mutagenesis_len.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mutagenesis_len.tex}}
    \caption*{\textbf{Time} (sec)}
    \label{fig:2third4}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mutagenesis_random.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mutagenesis_random.tex}}
    \caption*{\textbf{Time} (sec)}
    \label{fig:2third5}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mutagenesis_random.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mutagenesis_sampling.tex}}
    \caption*{\textbf{Time} (sec)}
    \label{fig:2third6}
\end{subfigure}
\else\QUICK
\fi
\caption{Different scheme reduction methods on all the downstream tasks.
\label{fig:selected_graphs_time_acc_vis}}
\end{figure*}
%end 9 last mutagenesis

























%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
















% \begin{figure*}[h!]
% %1 world
% \centering
% \rotatebox[origin=t]{90}{Acc-World}
% \begin{subfigure}{0.155\textwidth}
%     \caption*{\textbf{k\_var}}
%     \includegraphics[width=\textwidth]{plots/temp/world_kvar.png}
%     %\caption{Time}
%     \label{fig:first}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.155\textwidth}
%     \caption*{\textbf{1ep}}
%     \includegraphics[width=\textwidth]{plots/temp/world_ent.png}
%     %\caption{Time}
%     \label{fig:second}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.155\textwidth}
%     \caption*{\textbf{ent}}
%     \includegraphics[width=\textwidth]{plots/temp/world_1epoch.png}
%     %\caption{Time}
%     \label{fig:third}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.155\textwidth}
%     \includegraphics[width=\textwidth]{plots/temp/world_len.png}
%     %\caption{Time}
%     \label{fig:third4}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.155\textwidth}
%     \includegraphics[width=\textwidth]{plots/temp/world_random.png}
%     %\caption{Time}
%     \label{fig:third5}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.155\textwidth}
%     \includegraphics[width=\textwidth]{plots/temp/world_random.png}
%     %\caption{Time}
%     \label{fig:third6}
% \end{subfigure}
% %\caption{Subreferences in \LaTeX.}





% % \end{figure*}
% \centering
% \rotatebox[origin=t]{90}{Acc-World}
% \begin{subfigure}{0.155\textwidth}
%     \caption*{\textbf{k\_var}}
%     \includegraphics[width=\textwidth]{plots/temp/world_kvar.png}
%     %\caption{Time}
%     \label{fig:22first}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.155\textwidth}
%     \caption*{\textbf{1ep}}
%     \includegraphics[width=\textwidth]{plots/temp/world_1epoch.png}
%     %\caption{Time}
%     \label{fig:22second}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.155\textwidth}
%     \caption*{\textbf{ent}}
%     \includegraphics[width=\textwidth]{plots/temp/world_ent.png}
%     %\caption{Time}
%     \label{fig:22third}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.155\textwidth}
%     \includegraphics[width=\textwidth]{plots/temp/world_ent.png}
%     %\caption{Time}
%     \label{fig:22third4}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.155\textwidth}
%     \includegraphics[width=\textwidth]{plots/temp/world_ent.png}
%     %\caption{Time}
%     \label{fig:22third5}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.155\textwidth}
%     \includegraphics[width=\textwidth]{plots/temp/world_ent.png}
%     %\caption{Time}
%     \label{fig:22third6}
% \end{subfigure}
% %\caption{Subreferences in \LaTeX.}

% \centering
% \rotatebox[origin=t]{90}{Acc-World}
% \begin{subfigure}{0.155\textwidth}
%     \caption*{\textbf{k\_var}}
%     \includegraphics[width=\textwidth]{plots/temp/world_kvar.png}
%     %\caption{Time}
%     \label{fig:3first}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.155\textwidth}
%     \caption*{\textbf{1ep}}
%     \includegraphics[width=\textwidth]{plots/temp/world_1epoch.png}
%     %\caption{Time}
%     \label{fig:3second}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.155\textwidth}
%     \caption*{\textbf{ent}}
%     \includegraphics[width=\textwidth]{plots/temp/world_ent.png}
%     %\caption{Time}
%     \label{fig:3third}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.155\textwidth}
%     \includegraphics[width=\textwidth]{plots/temp/world_ent.png}
%     %\caption{Time}
%     \label{fig:3third4}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.155\textwidth}
%     \includegraphics[width=\textwidth]{plots/temp/world_ent.png}
%     %\caption{Time}
%     \label{fig:3third5}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.155\textwidth}
%     \includegraphics[width=\textwidth]{plots/temp/world_ent.png}
%     %\caption{Time}
%     \label{fig:3third6}
% \end{subfigure}
% %\caption{Subreferences in \LaTeX.}
% % \begin{figure*}[h!]
% % \centering





% \rotatebox[origin=t]{90}{Acc-Mutagenesis}
% \begin{subfigure}{0.155\textwidth}
%     \includegraphics[width=\textwidth]{plots/temp/world_kvar.png}
%     \caption*{Time}
%     \label{fig:2first}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.155\textwidth}
%     \includegraphics[width=\textwidth]{plots/temp/world_1epoch.png}
%     \caption*{Time}
%     \label{fig:2second}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.155\textwidth}
%     \includegraphics[width=\textwidth]{plots/temp/world_ent.png}
%     \caption*{Time}
%     \label{fig:2third}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.155\textwidth}
%     \includegraphics[width=\textwidth]{plots/temp/world_ent.png}
%     \caption*{Time}
%     \label{fig:2third4}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.155\textwidth}
%     \includegraphics[width=\textwidth]{plots/temp/world_ent.png}
%     \caption*{Time}
%     \label{fig:2third5}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.155\textwidth}
%     \includegraphics[width=\textwidth]{plots/temp/world_ent.png}
%     \caption*{Time}
%     \label{fig:2third6}
% \end{subfigure}
        
% \caption{Different scheme reduction methods on few downstream tasks.}
% \label{fig:selected_graphs_time_acc_vis}
% \end{figure*}

==> plots/mega_figure_split2.tex <==
\begin{figure*}
\ifx\QUICK\undefined
%begin 1 world
\centering
\rotatebox[origin=t]{90}{\small~\textbf{World}}
\begin{subfigure}{0.155\textwidth}
    \caption*{\textbf{\kvar}}
    %\includegraphics[width=\textwidth]{plots/world_k_var.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/world_k_var.tex}}
    %\caption{Time}
    \label{fig:first}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    \caption*{\textbf{\mi}}
    %\includegraphics[width=\textwidth]{plots/world_ent.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/world_MI.tex}}
    %\caption{Time}
    \label{fig:second}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    \caption*{\textbf{\oneepoch}}
    %\includegraphics[width=\textwidth]{plots/world_1ep.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/world_1ep.tex}}
    %\caption{Time}
    \label{fig:third}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    \caption*{\textbf{\length}}
    %\includegraphics[width=\textwidth]{plots/world_len.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/world_len.tex}}
    %\caption{Time}
    \label{fig:third4}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    \caption*{\textbf{\random}}
    %\includegraphics[width=\textwidth]{plots/world_random.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/world_random.tex}}
    %\caption{Time}
    \label{fig:third5}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    \caption*{\textbf{\sampling}}
    %\includegraphics[width=\textwidth]{plots/world_sampling.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/world_sampling.tex}}
    %\caption{Time}
    \label{fig:third6}
\end{subfigure}
%end 1 world






%begin 2 genes
\centering
\rotatebox[origin=t]{90}{\small~\textbf{Genes}}
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/genes_k_var.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/genes_k_var.tex}}
    %\label{fig:first}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/genes_ent.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/genes_MI.tex}}
    %\label{fig:second}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/genes_1ep.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/genes_1ep.tex}}
    %\label{fig:third}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/genes_len.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/genes_len.tex}}
    %\label{fig:third4}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/genes_random.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/genes_random.tex}}
    %\label{fig:third5}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/genes_sampling.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/genes_sampling.tex}}
    %\label{fig:third6}
\end{subfigure}
%end 2 genes






%begin 3 mondial_religion
\centering
\rotatebox[origin=t]{90}{\small~\textbf{M-Religion}} %Acc-mondial_religion
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_religion_k_var.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_religion_k_var.tex}}
    %\label{fig:first}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_religion_ent.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_religion_MI}}
    %\label{fig:second}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_religion_1ep.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_religion_1ep.tex}}
    %\label{fig:third}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_religion_len.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_religion_len.tex}}
    %\label{fig:third4}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_religion_random.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_religion_random.tex}}
    %\label{fig:third5}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_religion_sampling.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_religion_sampling.tex}}
    %\label{fig:third6}
\end{subfigure}
%end 3 mondial_religion






%begin 4 mondial_continent
\centering
\rotatebox[origin=t]{90}{\small~\textbf{M-Continent}} %
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_continent_k_var.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_continent_k_var.tex}}
    \caption*{\textbf{Time} (sec)}
    %\label{fig:first}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_continent_ent.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_continent_MI}}
    \caption*{\textbf{Time} (sec)}
    %\label{fig:second}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_continent_1ep.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_continent_1ep.tex}}
    \caption*{\textbf{Time} (sec)}
    %\label{fig:third}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_continent_len.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_continent_len.tex}}
    \caption*{\textbf{Time} (sec)}
    %\label{fig:third4}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_continent_random.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_continent_random.tex}}
    \caption*{\textbf{Time} (sec)}
    %\label{fig:third5}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_continent_random.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_continent_sampling.tex}}
    \caption*{\textbf{Time} (sec)}
    %\label{fig:third6}
\end{subfigure}
%end 4 mondial_continent

\caption{The performance on the downstream task as a function of time for different ratios of targeted walk schemes used for training. More precisely, in the end of each training epoch of \forward we record the time (x-axis) and the accuracy of the downstream task (y-axis).
\label{fig:selected_graphs_time_acc_vis1}}

\end{figure*}

























%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%









\begin{figure*}
%begin 5 mondial_inflation
\centering
\rotatebox[origin=t]{90}{\small~\textbf{M-Inflation}} %Acc-mondial_inflation
\begin{subfigure}{0.155\textwidth}
    \caption*{\textbf{\kvar}}
    %\includegraphics[width=\textwidth]{plots/mondial_inflation_k_var.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_inflation_k_var.tex}}
    %\label{fig:first}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    \caption*{\textbf{\mi}}
    %\includegraphics[width=\textwidth]{plots/mondial_inflation_ent.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_inflation_MI}}
    %\label{fig:second}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    \caption*{\textbf{\oneepoch}}
    %\includegraphics[width=\textwidth]{plots/mondial_inflation_1ep.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_inflation_1ep.tex}}
    %\label{fig:third}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    \caption*{\textbf{\length}}
    %\includegraphics[width=\textwidth]{plots/mondial_inflation_len.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_inflation_len.tex}}
    %\label{fig:third4}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    \caption*{\textbf{\random}}
    %\includegraphics[width=\textwidth]{plots/mondial_inflation_random.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_inflation_random.tex}}
    %\label{fig:third5}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    \caption*{\textbf{\sampling}}
    %\includegraphics[width=\textwidth]{plots/mondial_inflation_sampling.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_inflation_sampling.tex}}
    %\label{fig:third6}
\end{subfigure}
%end 5 mondial_inflation






%begin 6 hepatitis
\centering
\rotatebox[origin=t]{90}{\small~\textbf{Hepatitis}}
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/hepatitis_k_var.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/hepatitis_k_var.tex}}
    %\label{fig:first}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/hepatitis_ent.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/hepatitis_MI}}
    %\label{fig:second}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/hepatitis_1ep.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/hepatitis_1ep.tex}}
    %\label{fig:third}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/hepatitis_len.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/hepatitis_len.tex}}
    %\label{fig:third4}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/hepatitis_random.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/hepatitis_random.tex}}
    %\label{fig:third5}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/hepatitis_sampling.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/hepatitis_sampling.tex}}
    %\label{fig:third6}
\end{subfigure}
%end 6 hepatitis






%begin 7 mondial_infant-mortality
\centering
\rotatebox[origin=t]{90}{\small~\textbf{M-Infant Mort.}} %Acc-mondial_infant-mortality
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_infant-mortality_k_var.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_infant-mortality_k_var.tex}}
    %\label{fig:first}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_infant-mortality_ent.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_infant-mortality_MI}}
    %\label{fig:second}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_infant-mortality_1ep.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_infant-mortality_1ep.tex}}
    %\label{fig:third}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_infant-mortality_len.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_infant-mortality_len.tex}}
    %\label{fig:third4}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_infant-mortality_random.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_infant-mortality_random.tex}}
    %\label{fig:third5}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_infant-mortality_sampling.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_infant-mortality_sampling.tex}}
    %\label{fig:third6}
\end{subfigure}
%end 7 mondial_infant-mortality






%begin 8 mondial_GDP
\centering
\rotatebox[origin=t]{90}{\small~\textbf{M-GDP}} %Acc-mondial_GDP
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_GDP_k_var.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_GDP_k_var.tex}}
    %\label{fig:first}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_GDP_ent.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_GDP_MI}}
    %\label{fig:second}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_GDP_1ep.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_GDP_1ep.tex}}
    %\label{fig:third}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_GDP_len.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_GDP_len.tex}}
    %\label{fig:third4}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_GDP_random.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_GDP_random.tex}}
    %\label{fig:third5}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mondial_GDP_sampling.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mondial_GDP_sampling.tex}}
    %\label{fig:third6}
\end{subfigure}
%end 8 mondial_GDP







%begin 9 last mutagenesis
\rotatebox[origin=t]{90}{\small~\textbf{Mutagenesis}} 
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mutagenesis_k_var.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mutagenesis_k_var.tex}}
    \caption*{\textbf{Time} (sec)}
    \label{fig:2first}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mutagenesis_1ep.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mutagenesis_MI.tex}}
    \caption*{\textbf{Time} (sec)}
    \label{fig:2second}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/empty.png}  % mutagenesis_entropy
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mutagenesis_1ep}}
    \caption*{\textbf{Time} (sec)}
    \label{fig:2third}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mutagenesis_len.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mutagenesis_len.tex}}
    \caption*{\textbf{Time} (sec)}
    \label{fig:2third4}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mutagenesis_random.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mutagenesis_random.tex}}
    \caption*{\textbf{Time} (sec)}
    \label{fig:2third5}
\end{subfigure}
\hfill
\begin{subfigure}{0.155\textwidth}
    %\includegraphics[width=\textwidth]{plots/mutagenesis_random.png}
    \resizebox{\linewidth}{!}{\input{plots/pgf_plots/mutagenesis_sampling.tex}}
    \caption*{\textbf{Time} (sec)}
    \label{fig:2third6}
\end{subfigure}
\else\QUICK
\fi
\caption{The performance on the downstream task as a function of time for different ratios of targeted walk schemes used for training. More precisely, in the end of each training epoch of \forward we record the time (x-axis) and the accuracy of the downstream task (y-axis).
\label{fig:selected_graphs_time_acc_vis2}}
\end{figure*}




% \begin{figure*}[h!]
% %1 world
% \centering
% \rotatebox[origin=t]{90}{Acc-World}
% \begin{subfigure}{0.155\textwidth}
%     \caption*{\textbf{k\_var}}
%     \includegraphics[width=\textwidth]{plots/temp/world_kvar.png}
%     %\caption{Time}
%     \label{fig:first}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.155\textwidth}
%     \caption*{\textbf{1ep}}
%     \includegraphics[width=\textwidth]{plots/temp/world_ent.png}
%     %\caption{Time}
%     \label{fig:second}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.155\textwidth}
%     \caption*{\textbf{ent}}
%     \includegraphics[width=\textwidth]{plots/temp/world_1epoch.png}
%     %\caption{Time}
%     \label{fig:third}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.155\textwidth}
%     \includegraphics[width=\textwidth]{plots/temp/world_len.png}
%     %\caption{Time}
%     \label{fig:third4}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.155\textwidth}
%     \includegraphics[width=\textwidth]{plots/temp/world_random.png}
%     %\caption{Time}
%     \label{fig:third5}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.155\textwidth}
%     \includegraphics[width=\textwidth]{plots/temp/world_random.png}
%     %\caption{Time}
%     \label{fig:third6}
% \end{subfigure}
% %\caption{Subreferences in \LaTeX.}





% % \end{figure*}
% \centering
% \rotatebox[origin=t]{90}{Acc-World}
% \begin{subfigure}{0.155\textwidth}
%     \caption*{\textbf{k\_var}}
%     \includegraphics[width=\textwidth]{plots/temp/world_kvar.png}
%     %\caption{Time}
%     \label{fig:22first}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.155\textwidth}
%     \caption*{\textbf{1ep}}
%     \includegraphics[width=\textwidth]{plots/temp/world_1epoch.png}
%     %\caption{Time}
%     \label{fig:22second}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.155\textwidth}
%     \caption*{\textbf{ent}}
%     \includegraphics[width=\textwidth]{plots/temp/world_ent.png}
%     %\caption{Time}
%     \label{fig:22third}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.155\textwidth}
%     \includegraphics[width=\textwidth]{plots/temp/world_ent.png}
%     %\caption{Time}
%     \label{fig:22third4}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.155\textwidth}
%     \includegraphics[width=\textwidth]{plots/temp/world_ent.png}
%     %\caption{Time}
%     \label{fig:22third5}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.155\textwidth}
%     \includegraphics[width=\textwidth]{plots/temp/world_ent.png}
%     %\caption{Time}
%     \label{fig:22third6}
% \end{subfigure}
% %\caption{Subreferences in \LaTeX.}

% \centering
% \rotatebox[origin=t]{90}{Acc-World}
% \begin{subfigure}{0.155\textwidth}
%     \caption*{\textbf{k\_var}}
%     \includegraphics[width=\textwidth]{plots/temp/world_kvar.png}
%     %\caption{Time}
%     \label{fig:3first}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.155\textwidth}
%     \caption*{\textbf{1ep}}
%     \includegraphics[width=\textwidth]{plots/temp/world_1epoch.png}
%     %\caption{Time}
%     \label{fig:3second}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.155\textwidth}
%     \caption*{\textbf{ent}}
%     \includegraphics[width=\textwidth]{plots/temp/world_ent.png}
%     %\caption{Time}
%     \label{fig:3third}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.155\textwidth}
%     \includegraphics[width=\textwidth]{plots/temp/world_ent.png}
%     %\caption{Time}
%     \label{fig:3third4}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.155\textwidth}
%     \includegraphics[width=\textwidth]{plots/temp/world_ent.png}
%     %\caption{Time}
%     \label{fig:3third5}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.155\textwidth}
%     \includegraphics[width=\textwidth]{plots/temp/world_ent.png}
%     %\caption{Time}
%     \label{fig:3third6}
% \end{subfigure}
% %\caption{Subreferences in \LaTeX.}
% % \begin{figure*}[h!]
% % \centering





% \rotatebox[origin=t]{90}{Acc-Mutagenesis}
% \begin{subfigure}{0.155\textwidth}
%     \includegraphics[width=\textwidth]{plots/temp/world_kvar.png}
%     \caption*{Time}
%     \label{fig:2first}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.155\textwidth}
%     \includegraphics[width=\textwidth]{plots/temp/world_1epoch.png}
%     \caption*{Time}
%     \label{fig:2second}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.155\textwidth}
%     \includegraphics[width=\textwidth]{plots/temp/world_ent.png}
%     \caption*{Time}
%     \label{fig:2third}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.155\textwidth}
%     \includegraphics[width=\textwidth]{plots/temp/world_ent.png}
%     \caption*{Time}
%     \label{fig:2third4}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.155\textwidth}
%     \includegraphics[width=\textwidth]{plots/temp/world_ent.png}
%     \caption*{Time}
%     \label{fig:2third5}
% \end{subfigure}
% \hfill
% \begin{subfigure}{0.155\textwidth}
%     \includegraphics[width=\textwidth]{plots/temp/world_ent.png}
%     \caption*{Time}
%     \label{fig:2third6}
% \end{subfigure}
        
% \caption{Different scheme reduction methods on few downstream tasks.}
% \label{fig:selected_graphs_time_acc_vis}
% \end{figure*}

==> section_related_work.tex <==
{\color{red}
\section{Related Work}\label{sec:related}
%\ylinline{Several related works to look when writing the introduction (in comment)}
\begin{comment}
%What is an Embedding:
Standard machine learning algorithms assume representations of their input data as numerical vectors. Using these algorithms for the analysis of non-numerical data requires \emph{embeddings} of these data.
Embedding is the process of converting high-dimensional data to low-dimensional data (typically) in the form of a finite dimensional Euclidean vector in such a way that the two entities are semantically similar.
Predominantly, similar entities should be mapped to vectors that are geometrically close, and vice versa.
An embedding can be learned once and reused across different models.

%Examples of Embedding:
In some modalities, the input comes with a useful embedding to begin with; for example, an image can be represented by the RGB intensities of its pixels. In others, semantic-aware embeddings have to be devised, and indeed have been devised, such as  \wordtovec~\cite{miksutche+13} and \glove~\cite{DBLP:conf/emnlp/PenningtonSM14} for words of natural language~\cite{DBLP:conf/icml/LeM14}, \nodetovec\ for the nodes of a graph~\cite{10.1145/2939672.2939754}, \transe~\cite{borusugar+13} for the entities of a knowledge graph, and \moltovec~\cite{DBLP:journals/jcisd/JaegerFT18} for molecule structures.

%Databases Embeddings:
Various approaches have been proposed for obtaining embeddings in databases. 
One is to concatenate predefined embeddings of the attribute values (which are, e.g., words or quantities)~\cite{DBLP:conf/sigmod/MudgalLRDPKDAR18,DBLP:journals/pvldb/EbraheemTJOT18} or permutations over the list of values~\cite{DBLP:conf/sigmod/CappuzzoPT20}. 
Another approach views the tuples as text documents and applies word and document embeddings~\cite{10.1145/3076246.3076251}. 

%Now we describe 2 related works to this reasurch: FoRWaRD and EmbDI
More recently, Cappuzzo, Papotti and Thirumuruganathan~\cite{DBLP:conf/sigmod/CappuzzoPT20} studied the approach of transforming the database into a graph and applying a node embedding over this graph. 
They use a heterogeneous graph with three types of nodes. \e{Token} nodes which correspond to the unique values found in the dataset. \e{Record Id} nodes (RIDs) which represent a unique token for each tuple.
And \e{Column Id} nodes (CIDs) which represent a unique token for each column/attribute. These nodes are connected by edges based on the structural relationships in the schema.

Arguably, an important advantage of the graph approach is that it utilizes information that should be highly relevant to the semantics of the data and is freely available in databases: the \e{structure} of the data. (See~\cite{DBLP:conf/pods/Grohe20} for a recent essay on embeddings for structured data.)  
For example, we can infer considerable information about a tuple with apparently meaningless values, such as internal codes, by looking at the tuples that are referenced by this tuple and their attributes. 
It has been shown to be useful in the general context of machine learning~\cite{DBLP:conf/cidm/SchulteBCBX13,shah2017key}. 
After creating the graph, they produce a large number of random walks on the graph (using \nodetovec~\cite{10.1145/2939672.2939754} or another embedding generation algorithm) and gather them in a training corpus where each random walk will correspond to a sentence.
From this collection of sentences the different embeddings are created using an embedding algorithm such as word2vec, GloVe, fastText, and so on. 
We can think of this method as a reduction from the database embedding to embedding over the sentences produced by the random walks over the graph.


We are aware of only one embedding technique that directly uses the most common way of referencing tuples, namely foreign-key references. This embedding technique is presented in FoRWaRD~\cite{DBLP:journals/corr/abs-2103-06766}.
The FoRWaRD algorithm utilizes these for the sake of high-quality tuple embedding. It considers random walks over database facts, where the transition from one fact to another follows a pattern (or scheme) of FK (forward or backward) references. 
%
Intuitively, FoRWaRD embeddings aim to model the
similarity of the random walk destinations.
% $d_{s,f}$ for all $R$-facts $f$ and all walk schemes $s\in \mathcal{T}(R, \ell_\text{max})$ up to a certain walk length $\ell_\text{max}$ with one vector representation $\phi$. It involves also training an additional matrix that allows it to encode multiple similarity measures (one for each $(s,A)$) into one vector embedding for tuples. 


Generally, in most of the algorithms, the embeddings creation procedure is similar.
The embeddings creation procedure can be divided into two main steps:
\begin{itemize}
    \item \emph{Random walk collection:} Collect a corpus of sentences that capture the structure of the database. It can be done by sampling random walks over the database or the graph which represents the database. The walks can %usually must
    follow foreign keys and shared attribute values of tuples.
    \item \emph{Analysis of random walks:} From the collection of sentences\footnote{note that we need to compute it only once.} we can create different embeddings. One way to do so is 
    by analyzing the sentences as natural language sentences,
    using an embedding algorithm such as word2vec, GloVe, fastText, and so on. Another way to create the embeddings is to model the similarity of the random walk destinations, as presented in \forward.
\end{itemize}
Finally we can evaluate the quality of the embeddings, and compare between two of them using downstream learning tasks on the relational data.

% %why embdi and forward could be better and more scheme aware
% In \embdi~\cite{DBLP:conf/sigmod/CappuzzoPT20} the random walks do not follow a scheme at all. 
% When creating the corpus of random walks (sentences) from the graph, we lose a lot of information about the relations structure.
% As oppose to random walks on a graph, where in the database there is plenty of metadata. For example, the names of the relations or the name of the attributes.
% When traversing over the database over a specific walk pattern, all the sentences have the same structure. Our hypothesis is that in this scenario, an embedding algorithm can better guess the next "word" in the sentence. 
% For example, if all the sentences have the same structure, where the second "word" is from a specific relation. An algorithm that learns the embedding by guessing words in the sentence, will have more information about the second word (for example the relation it comes from). As a result, the algorithm will have a better guess of that "word", in contrast to a scenario where the second "word" in each sentence could be taken from many different relations.
% In addition, there exist sentences in the corpus without any semantic meaning that may add noise to the input of the embedding algorithms, and if we remove them, it will benefit the quality of the embeddings. For example, a walk that connects a phone number to it's owner's id. 
% Hence, we argue %think
% that devising algorithms that are better aware of the walk schemes, and traversing on them will be beneficial to the quality evaluation of the embeddings and \embdi~\cite{DBLP:conf/sigmod/CappuzzoPT20} did not refer to that at all.

% FoRWaRD~\cite{DBLP:journals/corr/abs-2103-06766} tune the embeddings over all walk schemes
% up to a certain walk length $\ell_\text{max}$. It is an arbitrary choice to use all the walk schemes, and in the article there was no reference to the influence of choosing all the walk schemes on the quality evaluation of the embeddings. Our assumption is that as a result of this choice there might be some walk schemes which damage the quality of the embeddings. The single embedding tries to take into account all the walk schemes, instead of focusing (minimizing the loss) over fewer, more important walk schemes.
% For that reason, the embedding might be better tuned on a noisy (or meaningless) scheme, but not on the important schemes, with semantic a meaning.
\ylinline{write}
\end{comment}
}


==> section_research_goals.tex <==
\section{Research Goals}
The main goal of this research is making the embedding algorithms better aware of the walk schemes in order to considerably improve the quality of solutions for downstream tasks such as column prediction, data imputation, and entity linkage/resolution. 
%-----------------
%The main objective of the study is to to improve the quality evaluation of relational database embeddings by making algorithms more aware on walk schemes.
Our planned research consists of three parts:
\begin{enumerate}
    \item Investigate the importance and impact of the walk schemes on the quality evaluation of the embeddings. 
    \item Optimize the selection of the walk schemes and improve the embeddings quality of existing algorithms, such as \forward and \embdi.
    %\item Devise new algorithms for selecting beneficial walk schemes. In particular, we plan to come up with algorithms that are more aware on walk schemes. 
    \item Better incorporate the walk schemes in the embedding algorithms, for instance, introduce parameters that allow weighting the %paths 
    random walks according to their schemes. 
%In addition, optimize the selection of the walk schemes.
\end{enumerate}

\subsection{Understanding the Impact of the Walk Schemes}
We will first study the impact of the walk schemes on the quality evaluation of the embeddings that are generated. 

%\subsection{Impact of Walk Schemes Length on the Embeddings}
\emph{Impact of Walk Schemes Length on the Embeddings.}
Our first research question is whether the length of these walk schemes has an effect on the quality evaluation of the embeddings? 

%maybe put in the experimental plan part:
For instance, the \forward algorithm presents random walks over database facts, where the transition from one fact to another follows a pattern (or scheme) of FK (forward or backward) references. The tuple embeddings are based on all the schemes up to the maximum walk length hyperparameter $l_{max}$. We will check the importance of this walk schemes length on the embeddings.


%\subsection{The importance of the Number Of Walk Schemes}
\emph{The importance of the Number Of Walk Schemes.}
Our second research question is how does changing the number of schemes affect the quality evaluation of the embeddings produced?
In particular, if enlarging %increasing
the number of different schemes increases or decreases quality evaluation of the embeddings. For example, does removing half of the schemes before creating the random walks affect the quality evaluation of the embeddings (produced by \forward and \embdi)?

%maybe put in the experimental plan part:
For instance, as explained above, the \forward algorithm creates the tuple embeddings based on all the schemes up to the maximum walk length hyper parameter  $l_{max}$. We will check the impact of different quantity of walk schemes on the embeddings.


\subsection{Optimizing the Selection of the Schemes}
We would like to optimize the selection of the "best" subset of schemes that maximizes the quality evaluation of the embeddings.

%\textbf{The effect of meaningless walk schemes.} Our third research question is if there are schemes that damage the quality evaluation of the embedding. More specifically, if including them in the random walks generating part in the \forward algorithm damage the quality evaluation of the embedding. In, particular, if there are some schemes that don't have a semantic meaning with respect to the structure of the relational database. And tuning the embeddings in the \forward optimization part (when using gradient descent) with them, adds "noise" to the random walks, thus leading the embeddings to not train properly.
%
\emph{The effect of meaningless walk schemes.} Our third research question is whether schemes that damage the quality evaluation of the embedding exist. More specifically, does including them in the random walks generating part in the \forward algorithm damage the quality evaluation of the embedding. In particular, are there schemes that do not have a semantic meaning with respect to the structure of the relational database. 
We believe that tuning the embeddings in the \forward optimization part (when using gradient descent) with these schemes, adds "noise" to the random walks, leading the embeddings to not train properly.
%

\emph{Walk Schemes Subset Selection.} Our fourth research question is whether we can determine during the training stage what schemes are beneficial to the downstream task in order to remove the least helpful (or most "damaging") schemes before training the embeddings, and how.

We want to propose a method that optimizes the selecting of the subset of beneficial walk schemes.
%Intuition: If we think about the schemes we use as "features", we would like to do a Recursive Feature Elimination (RFE) in such a way that in each iteration we remove the least beneficial scheme. In order to do so, we need a way to compare between 2 schemes and determine which one is more relevant for the downstream task. 
In general, we can either throw the unwanted schemes before the embeddings are tuned, afterwards and run the optimization part again or creating an architecture that gives weights to the different schemes (which will give different significance to each scheme).  




